MADGEN: Mass-Spec attends to De Novo Molecular generation

The annotation (assigning structural chemical identities) of MS/MS spectra remains a significant challenge due to the enormous molecular diversity in biological samples and the limited scope of reference databases. Currently, the vast majority of spectral measurements remain in the "dark chemical space" without structural annotations. To improve annotation, we propose MADGEN (Mass-spec Attends to De Novo Molecular GENeration), a scaffold-based method for de novo molecular structure generation guided by mass spectrometry data. MADGEN operates in two stages: scaffold retrieval and spectra-conditioned molecular generation starting with the scaffold. In the first stage, given an MS/MS spectrum, we formulate scaffold retrieval as a ranking problem and employ contrastive learning to align mass spectra with candidate molecular scaffolds. In the second stage, starting from the retrieved scaffold, we employ the MS/MS spectrum to guide an attention-based generative model to generate the final molecule. Our approach constrains the molecular generation search space, reducing its complexity and improving generation accuracy. We evaluate MADGEN on three datasets (NIST23, CANOPUS, and MassSpecGym) and evaluate MADGEN's performance with a predictive scaffold retriever and with an oracle retriever. We demonstrate the effectiveness of using attention to integrate spectral information throughout the generation process to achieve strong results with the oracle retriever.

==> sections/introduction.tex <==
\section{Introduction}
Metabolomics, the measurement and identification of small molecules in biological samples, plays a critical role in numerous fields, including drug discovery, disease diagnosis, and environmental science. By analyzing the molecular composition of complex biological samples, metabolomics provides insights into cellular processes, metabolic pathways, and the effects of environmental changes on biological systems. Tandem mass spectrometry (MS/MS) has emerged as a powerful, widely used analytical technique that can separate and fragment molecules within a biological sample, thus producing rich spectra that can be further analyzed to annotate the measurements within the sample \citep{kind2018identification}.  

Despite the utility of MS/MS techniques in metabolomics, annotation (assigning a chemical structural identity to a measured spectrum) remains a significant challenge. 
Currently, most MS/MS spectra cannot be linked to known molecular structures due to the vast chemical diversity in biological samples and the limited scope of reference databases. Spectral databases that catalogue molecules and their measured spectra, e.g., MoNA\citep{MoNA} and GNPS\citep{aron2020reproducible},  are used for identifying a close match to the measured spectra. However, such databases remain relatively small. Molecular databases such as PubChem\citep{kim2016pubchem} and KEGG\citep{kanehisa2021kegg} are often utilized to provide \textit{candidate} molecular structures when using computational methods such as SIRIUS \citep{duhrkop2019sirius}, MLP or GNN-based approaches \citep{wei2019rapid}\citep{zhu2020using} to predict the molecular structure that most likely matches the measured spectrum. Despite the success of these tools and the large size of such databases, the "dark chemical space" of unknown molecules remains large.  
The lack of information on these unknown molecules hinders the  identification and characterization of molecules,  making it challenging to link them to known molecular structures \citep{atanasov2021natural, patti2012metabolomics}. 

De novo molecular structure prediction from mass spectra is a promising approach to overcome the limitations of database-dependent methods. Instead of relying on existing libraries, de novo techniques aim to generate molecular structures directly from spectral data, making it possible to explore previously uncharacterized regions of chemical space. This capability is crucial for discovering novel metabolites and small molecules that play key roles in health, disease, and environmental processes.  

An insight in addressing this challenge is the potential use of scaffolds to simplify the structure prediction process. A scaffold, or core structure, is used widely in medicinal chemistry to represent core structures of bioactive compounds\citep{hu2016computational}. Such scaffolds can be modified with the addition of functional groups to enhance medicinal properties.  By focusing  on scaffold-based molecular generation in the context of annotation, we can reduce the complexity of structure generation and constrain the search space, making it more manageable and improving prediction accuracy. Once a scaffold is predicted, additional structural elements can be added to generate complete molecules that fit the observed spectral data.

% In this work, we propose a scaffold-based approach to de novo molecular structure prediction from MS/MS spectra. We formulate the problem as two tasks: scaffold prediction and scaffold-based molecular design. By guiding molecule generation with predicted scaffolds, we aim to improve the annotation of mass spectra and accelerate the discovery of novel compounds. This approach leverages the complementary strengths of mass spectrometry and advanced computational models to enhance the exploration of dark chemical space and drive innovations in metabolomics.
% \xh{contributions should be in here}


% \subsection{Our Contribution}

 We propose a scaffold-based approach to de novo molecular structure generation guided by mass spectrometry data, with a focus on evaluating performance both when the scaffold is known and when it is predicted. Our contributions are as follows:

\begin{itemize}
    \item We introduce a two-step framework that first predicts a  scaffold from MS/MS spectra, from which we then generate  the complete target molecular structure. Given the challenges in accurately predicting the scaffold, we report performance under two settings: using the correct scaffold and using the predicted scaffold. This comparison highlights the potential and limitations of scaffold prediction in de novo molecular generation.

    \item Our method leverages fragmentation patterns in MS/MS spectra to guide scaffold prediction. While scaffold prediction is not always accurate, integrating even partially correct scaffolds  reduces the complexity of de novo generation and constraints the search space to more plausible molecular structures.

    \item We benchmark our scaffold-based method against state-of-the-art models, such as MS2Mol and MSNovelist, using datasets the MassSpecGym. By evaluating performance with both  the correct scaffold and the predicted scaffold, we demonstrate the potential improvement that scaffold-guided generation offers, particularly in dark chemical space where novel compounds are common.

    \item The scaffold-based design also improves interpretability, as even predicted scaffolds serve as structural anchors for understanding the generated molecules. This interpretability is crucial for analyzing potential biological functions and chemical properties in practical applications.

    \item Our approach has broad applicability in metabolomics, drug discovery, and environmental analysis, where the discovery of novel metabolites, bioactive molecules, and uncharacterized compounds is essential.
    % The ability to compare results with correct and predicted scaffolds provides insights into the strengths and limitations of scaffold-based de novo generation.
\end{itemize}
